UniTraj: A Unified Framework for Scalable Vehicle Trajectory Prediction

Vehicle trajectory prediction has increasingly relied on data-driven solutions, but their ability to scale to different data domains and the impact of larger dataset sizes on their generalization remain under-explored. While these questions can be studied by employing multiple datasets, it is challenging due to several discrepancies, e.g., in data formats, map resolution, and semantic annotation types. To address these challenges, we introduce UniTraj, a comprehensive framework that unifies various datasets, models, and evaluation criteria, presenting new opportunities for the vehicle trajectory prediction field. In particular, using UniTraj, we conduct extensive experiments and find that model performance significantly drops when transferred to other datasets. However, enlarging data size and diversity can substantially improve performance, leading to a new state-of-the-art result for the nuScenes dataset. We provide insights into dataset characteristics to explain these findings. The code can be found here: https://github.com/vita-epfl/UniTraj

==> figs/kalman_difficulty.tex <==
\begin{figure}[t]
\centering
\trimbox{0.3cm 0cm 0cm 0cm}{ 
\begin{tikzpicture}[scale = 0.7]
  \begin{axis}[
    ybar=.3pt,
    width=1.08\linewidth,
    height=6cm,
    bar width=6pt,
    ylabel={\# trajectories (\%)},
    ylabel style={yshift=-7pt, align=center},
    xlabel={Kalman difficulty},
    xlabel style={yshift=4pt, align=center},
    ytick pos=left,
    xtick pos=bottom,
    xtick=data,
    xticklabels={0--5, 5--15, 15--25, 25--35, 35--45, 45--55, 55--65, 65--75}, %, 85, 95},
    %every x tick label/.append style={font=\footnotesize, rotate=45, anchor=east}, % Decrease font size for x tick labels and rotate
    every x tick label/.append style={font=\footnotesize}, % Decrease font size for x tick labels and rotate
    ymin=0,
    legend style={
      at={(0.99,0.99)},
      draw=none,
      anchor=north east,
      cells={anchor=west},
      legend columns=1,
      font=\footnotesize,
    },
    enlarge x limits={abs=0.45},
    legend image code/.code={%
        \draw[#1] (0cm,-0.1cm) rectangle (6pt,5pt);},
    ]
    
    % Dotted lines at y=10,20,30,40
    \draw[dotted] (axis cs:\pgfkeysvalueof{/pgfplots/xmin}, 10) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax}, 10);
    \draw[dotted] (axis cs:\pgfkeysvalueof{/pgfplots/xmin}, 20) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax}, 20);
    \draw[dotted] (axis cs:\pgfkeysvalueof{/pgfplots/xmin}, 30) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax}, 30);
    \draw[dotted] (axis cs:\pgfkeysvalueof{/pgfplots/xmin}, 40) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax}, 40);

    % Waymo bars
    \addplot[fill=Blue,draw=Blue!30!black] coordinates {
        (0, 23.952629169758517)
        (1, 24.611144221251667)
        (2, 21.142773679220554)
        (3, 15.996653629820514)
        (4, 9.446714336574939)
        (5, 3.7812939732733786)
        (6, 0.8821063091988663)
        (7, 0.1533644322320915)
%        (8, 0.027777741552241064)
%        (9, 0.005542507117231198)
    };

    % AV2 bars
     \addplot[fill=ForestGreen,draw=ForestGreen!30!black] coordinates {
        (0, 42.29571326493321)
        (1, 27.38459524471863)
        (2, 18.436942612622932)
        (3, 8.649833908788924)
        (4, 2.555459191743985)
        (5, 0.5563646479357236)
        (6, 0.10200018545488264)
        (7, 0.01581821057856469)
%        (8, 0.0027272776859594288)
%        (9, 0.0005454555371918858)
    };

    % NuScenes bars
    \addplot[fill=GreenYellow,draw=GreenYellow!30!black] coordinates {
        (0, 46.08954179783141)
        (1, 30.622595313046517)
        (2, 15.928646379853095)
        (3, 5.771248688352571)
        (4, 1.3326337880377754)
        (5, 0.24484085344526058)
        (6, 0.006995452955578873)
        (7, 0.0034977264777894365)
%        (8, 0.0)
%        (9, 0.0)
    };

    \legend{\waymo{}, Argoverse 2, nuScenes}
    
  % Overlay PNG images
  % Arrow pointing at a specific coordinate (example: (C, 20))
  \draw[black,->] (0.9,43) -- (0.4,43) node[midway, right]{};
  \begin{scope}
    \node[anchor=south west,inner sep=0,draw=black,line width=1pt] at (1,39) {\includegraphics[width=3.5cm]{figs/kalman_diff_1.PNG}};
  \end{scope}
  
  \draw[black,->] (2,30) -- (1.4,30) node[midway, right]{};
  \begin{scope}
    \node[anchor=south west,inner sep=0,draw=black,line width=1pt] at (2.1,24.5) {\includegraphics[width=3.5cm]{figs/kalman_diff_15.PNG}};
  \end{scope}
  
  \draw[black,->] (4.2,20) -- (2.4,20) node[midway, right]{};
  \begin{scope}
    \node[anchor=south west,inner sep=0,draw=black,line width=1pt] at (4.3,7) {\includegraphics[width=2cm]{figs/kalman_diff_18.PNG}};
  \end{scope}
  
  \end{axis}
  
\end{tikzpicture}
}
\caption{\textbf{Histogram of the Kalman Difficulty of trajectories.} To give a sense of the Kalman difficulty, we overlay random examples for three bins. The past trajectory is shown in red, future ground truth is shown in blue. The prediction from the Kalman filter is shown in magenta. The plot displays a clear trend where simpler scenarios are significantly more than challenging ones. \waymo{}, in particular, shows a relatively balanced distribution across scenarios.}
\label{fig:kalman}
\end{figure}


==> figs/trajectory_type.tex <==
\begin{figure}[t]
\centering
\trimbox{0.3cm 0cm 0cm 0cm}{ 
\begin{tikzpicture}[scale = 0.7]
  \begin{axis}[
    ybar=.3pt,
    width=1.08\linewidth,
    height=6cm,
    bar width=6pt,
    ylabel={\# trajectories (\%)},
    ylabel style={yshift=-7pt, align=center},
    %xlabel={Trajectory type},
    %xlabel style={yshift=4pt, align=center},
    ytick pos=left,
    xtick pos=bottom,
    xtick=data,
    xticklabels={Stationary, Straight, Straight Right, Straight Left, Right Turn, Left Turn, Left U-Turn, Right U-Turn},
    every x tick label/.append style={font=\footnotesize, rotate=45, anchor=east}, % Decrease font size for x tick labels and rotate
    ymin=0,
    legend style={
      at={(0.99,0.99)},
      draw=none,
      anchor=north east,
      cells={anchor=west},
      legend columns=1,
      font=\footnotesize,
    },
    enlarge x limits={abs=0.45},
    legend image code/.code={%
        \draw[#1] (0cm,-0.1cm) rectangle (6pt,5pt);},
    ]
    
    % Dotted lines at y=10,20,30,40
    \draw[dotted] (axis cs:\pgfkeysvalueof{/pgfplots/xmin}, 20) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax}, 20);
    \draw[dotted] (axis cs:\pgfkeysvalueof{/pgfplots/xmin}, 40) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax}, 40);
    \draw[dotted] (axis cs:\pgfkeysvalueof{/pgfplots/xmin}, 60) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax}, 60);
    
    % Waymo bars
    \addplot[fill=Blue,draw=Blue!30!black] coordinates {
          (0, 3.2596956361743965)
          (1, 54.013746235734985)
          (2, 3.7757510566071426)
          (3, 4.283858788075419)
          (4, 14.849766904081193)
          (5, 19.422518742392537)
          (6, 0.36325293465693204)
          (7, 0.03140970227739394)
    };
%
    % AV2 bars
    \addplot[fill=ForestGreen,draw=ForestGreen!30!black] coordinates {
          (0, 7.055467373577043)
          (1, 67.98394178898506)
          (2, 3.366551575548319)
          (3, 2.938914434389881)
          (4, 8.371106129283872)
          (5, 10.182563968298124)
          (6, 0.0692728532233695)
          (7, 0.032181876694321265)
    };
%
    % NuScenes bars
    \addplot[fill=GreenYellow,draw=GreenYellow!30!black] coordinates {
          (0, 2.738719832109129)
          (1, 70.05596362364463)
          (2, 4.0573627142357465)
          (3, 4.41063308849248)
          (4, 8.719832109129067)
          (5, 9.828611402588319)
          (6, 0.1259181532004197)
          (7, 0.06295907660020986)
    };

    \legend{\waymo{}, Argoverse 2, nuScenes}
  \end{axis}
\end{tikzpicture}
}
\caption{\textbf{Distribution of trajectory types across datasets.} It shows an imbalance across different types with straight being the most common trajectory type in the datasets. }
\label{fig:traj_type}
\end{figure}

